ADMM for ND Line Spectral Estimation using Grid-Free Compressive Sensing from Multiple Measurements with Applications to DOA Estimation

This paper is concerned with estimating unknown multi-dimensional frequencies from linear compressive measurements. This is accomplished by employing the recently proposed atomic norm minimization framework to recover these frequencies under a sparsity prior without imposing any grid restriction on these frequencies. To this end, we give a rigorous derivation of an iterative scheme called alternating direction of multipliers method, which is able to incorporate multiple compressive snapshots from a multi-dimensional superposition of complex harmonics. The key result here is how to formulate the objective function minimized by this scheme and its partial derivatives, which become hard to manage if the dimensionality of the frequencies is larger than 1. Moreover we demonstrate the performance of this approach in case of 3D line spectral estimation and 2D DOA estimation with a synthetic antenna array.

==> snippets/tex/clean_beamer.tex <==
\usepackage{amsmath}
\usepackage{amsfonts, amssymb, bm}

\beamertemplatenavigationsymbolsempty
\setbeamertemplate{section in toc}[sections numbered]
\setbeamertemplate{subsection in toc}[subsections numbered]
\setbeamersize{text margin left=7mm,text margin right=7mm}

\AtBeginSection[]
{
\begin{frame}
\begin{center}
\tableofcontents[currentsection]
\end{center}
\end{frame}
}

\setbeamertemplate{itemize item}{
    \color{black!50!white}$\blacktriangleright$\vspace{-10mm}
}

\setbeamertemplate{itemize subitem}{
    \color{black!30!white}$\blacktriangleright$
}

\setbeamertemplate{section in toc}{
    \color{gray} \Large \inserttocsection
}

\setbeamertemplate{frametitle}{
    \vspace{-2mm}
    \color{black} \hspace{2mm}\Large\bfseries\insertframetitle
    \vspace{2mm}
    \hrule
    \vspace{-10mm}
    }

\addtobeamertemplate{navigation symbols}{}{
    \usebeamerfont{date}\footnotesize\bfseries\color{black!75!white}
    \hspace{1em}
    \insertframenumber/\inserttotalframenumber
}

\usepackage[utf8]{inputenc}
\usepackage{color}
\linespread{1.5}
\usetheme{default}


==> snippets/tex/poster_skel/head.tex <==
\usepackage{psfrag}
\usepackage{array,makecell,booktabs}
\usepackage{filecontents}
\usepackage{longtable,tabularx}
\usepackage[size=a0,width=90,height=120,scale=1.4,orientation=portrait]{beamerposter}
\setbeamertemplate{navigation symbols}{}
\usepackage{tabularx}
\usepackage[none]{hyphenat}
\usepackage{bm}
\usepackage{multicol}
\usepackage{graphicx}
\usepackage{comment}
%\usepackage{natbib}
\usepackage{epstopdf}
\usepackage{booktabs}
\usepackage[font=small,labelfont=bf]{caption}
\usepackage{amsfonts, amsmath, amsthm, amssymb}
\usepackage{wrapfig}
\usepackage{wasysym}
\usepackage[justification=centering]{caption}
\usepackage[english]{babel}

\usepackage{tikz}
\usepackage{graphicx}
\usetikzlibrary{matrix,arrows,shapes,trees,fit}
\usetikzlibrary{calc,positioning,scopes,backgrounds}
\newif\ifoutertikznest
\outertikznestfalse
\usetikzlibrary{decorations.markings}

\newcommand{\tikzwidth}{0.48\textwidth}
\tikzstyle{lw} = [line width=3pt]

\usepackage{pgfplots}
\pgfplotsset{compat=newest}

\definecolor{box_white}{cmyk}{0.0361,0.0251,0.0166,0}
\definecolor{text_black}{cmyk}{0.7979,0.7417,0.6916,0.6554}
\definecolor{tui_orange_dark}{cmyk}{0,0.6,1,0} 
\definecolor{tui_orange_light}{cmyk}{0.0000,0.0876, 0.1474, 0.0157}
\definecolor{tui_green_dark}{cmyk}{1,0,0.5,0.2}
\definecolor{tui_green_light}{cmyk}{0.0576,0.0041, 0.0000, 0.0471} 
\definecolor{tui_blue_dark}{cmyk}{1.0000,0.5000,0.0000,0.6000}
\definecolor{tui_blue_light}{cmyk}{0.0920,0.0440,0.0000,0.0196}
\definecolor{tui_red_dark}{cmyk}{0.0000,1.0000,1.0000,0.2000}
\definecolor{tui_red_light}{cmyk}{0.0000,0.1107,0.1107,0.0078}

\pgfplotscreateplotcyclelist{tui_dark}{
{tui_orange_dark,mark=*},
{tui_green_dark,mark=square},
{tui_blue_dark,mark=triangle},
{tui_red_dark,mark=diamond},
}

\pgfplotsset{
    cycle list name=tui_dark,
}


\setbeamercolor{itemize item}{fg=tui_red_dark,bg=white}
\setbeamercolor{headline}{fg=black,bg=tui_blue_dark}
\setbeamercolor{title in headline}{fg=white}
\setbeamercolor{author in headline}{fg=white}
\setbeamercolor{institute in headline}{fg=white}
\setbeamercolor{logo in headline}{fg=black,bg=lightgray}
\setbeamercolor{footline}{fg=white,bg=tui_blue_dark}
\setbeamercolor{block}{fg=white,bg=umic_bg}
\setbeamercolor{caption name}{fg=tui_blue_dark}
\setbeamerfont{caption}{size=\small}

\setbeamercolor*{block body}{fg=text_black,bg=box_white}
\setbeamercolor*{block title}{fg=white,bg=tui_orange_dark}
\setbeamerfont{block title}{size=\normalsize,series=\bf}
\setbeamerfont{block body}{size=\normalsize}
\setbeamercolor{footlinecolor}{fg=white,bg=tui_blue_dark}
\setbeamertemplate{caption}[numbered]

%
% includes a logo wrapped around its own column
% scaling and path have to specified
%
\newcommand{\addlogo}[2]{
\begin{column}{.2\paperwidth}
\begin{center}
\topskip0pt
\vspace*{\fill}
\includegraphics[scale = #2]{#1}
\vspace*{\fill}
\end{center}
\end{column}
}

%
% put a light green frame around 
% something important within a text box
%
\newcommand{\frameIt}[2]{
	\begin{center}
	\vspace{13mm}
	\setbeamercolor*{block title}{fg=text_black,bg=tui_green_light}
	\setbeamercolor*{block body}{fg=text_black,bg=tui_green_light}
	\begin{minipage}{0.85\textwidth}
	\begin{block}{#1}\vspace{-8mm}\centering#2
	\end{block}
	\end{minipage}
	\end{center}
	\vspace{-10mm}
}

==> tex/multi_dim.tex <==
% !TEX root = ../main.tex

\subsection{Derivatives}

In contrast to \eqref{toep_single}, where $T(\bm u)$ is standard Toeplitz, now we consider the case, where we still want to approximately solve
%
\begin{align}
    \min_{t,\bm u, \bm x}
        \frac 12 \Norm{\bm \Gamma \bm x - \bm y}^2
        + \frac{\tau}{2}(t + \Real{u_{[1, \dots, 1]}}) \label{ML_ANM} \\
		\text{subject to} \quad
        \begin{bmatrix}
            \bm{T}_{(\bm{n},d)}(\bm u) & \bm x \\
            \bm x^\herm & t
        \end{bmatrix} \succeq \bm 0,  \notag
\end{align}
%
but now $\bm u \in \C^{n_1 \times \dots \times n_d}$ for $d \in \N$ and $\bm n = [n_1, \dots, n_d] \in \N^{n_1 \times \dots \times n_k}$ being a vector of dimension sizes and $\bm n_{1-} = [n_1,\dots, n_{d-1}]$ and $\bm n_{-1} = [n_2,\dots, n_d]$, where $\bm{T}_{(\bm{n},d)}(\bm u)$ is recursively defined as

\[\bm{T}_{(\bm{n},d)}(\bm u) =
\begin{bmatrix}
    \bm{T}_{(1,\bm{m}),\ell}        & \bm{T}_{(2,\bm{m}),\ell}
    & \dots  & \dots   & \bm{T}_{(n_1,\bm{m}),\ell}    \\
    \overline{\bm{T}_{(2,\bm{m}),\ell}}        & \bm{T}_{(1,\bm{m}),\ell}
    & \ddots & \dots   & \bm{T}_{(n_1 -1,\bm{m}),\ell}    \\
    \vdots                          & \ddots
    & \ddots & \ddots   & \vdots                            \\
    \overline{\bm{T}_{(n_1-1,\bm{m}),\ell}}    & \ddots
    & \ddots  & \ddots   & \bm{T}_{(2,\bm{m}),\ell}          \\
    \overline{\bm{T}_{(n_1,\bm{m}),\ell}}      & \overline{\bm{T}_{(n_1 - 1,\bm{m}),\ell}}
    & \dots  & \overline{\bm{T}_{(2,\bm{m}),\ell}}   & \bm{T}_{(1,\bm{m}),\ell}
\end{bmatrix} - \Diag(\Imag{u_{[1, \dots, 1]}}),
\]
where $\bm m = \bm n_{-1}$ and $\ell = d-1$. Here, we call the matrix $\bm{T}_{(\bm{n},d)}(\bm u)$ a Hermitian $d$-level Toeplitz. Note that in the case $d = 1$ we set $\bm T_{\bm n, 1}(\bm u) = \hat{T}(\bm u)$, where
\[\hat{T}(\bm u) = T(\bm u) + \Diag(\Imag{u_1})\]
and get the same result, as before. The inconvenience above enforced by the diagonal matrices stems from the fact that only the $d$-level Toeplitz matrix has to be Hermitian, but not its blocks, which only forces the main diagonal to be real and the recursion has to be written down a little bit strangely. Again, we would like to calculate the derivatives of interest
%
\[
\frac{\partial}{\partial \bm u} \langle \bm A, \bm{T}_{(\bm{n},d)}(\bm u) \rangle
\]
%
for a given Hermitian matrix $\bm A$. To this end, it is again useful to rewrite above inner product as a sum, as done in the chapter above. Similar to before for given $p \in \N$, we define $\bm{S}_{p}$ via
%
\begin{align}
  \bm S_{p} = \begin{bmatrix}
	0 & 1 & 0 & \ldots & 0 \\
	0 & 0 & 1 & \ldots & 0 \\
	\vdots & \ddots & \ddots & \ddots & \vdots \\
	0 & 0 & 0 & \ldots & 1 \\
	0 & 0 & 0 & \ldots & 0
\end{bmatrix} \in \R^{p \times p}, \quad \mbox{i.e.,} \; \left[\bm{S}_p\right]_{(k,\ell)} = 1 \; \mbox{if} \; \ell-k=1,
\end{align}
%
Note that $\bm{S}_p^d$ has ones on its $d$-th upper diagonal and zeros elsewhere. Moreover, for $d > 0$ we define $\bm S_p^{-d} = {\bm S_p^d}^\trans$ and $\bm S_p^0 = \bm I_p$. Now, we can rewrite
%
\begin{align}
\bm{T}_{(\bm{n},d)}(\bm u) = &
\sum\limits_{i_1 = 1}^{n_1}
\sum\limits_{i_2 = 1}^{n_2}
\dots
\sum\limits_{i_d = 1}^{n_d}
\left(
\bm S_{n_1}^{i_1-1} \otimes \dots \otimes \bm S_{n_d}^{i_d-1}
\right)
u_{[i_1, i_2, \dots, i_d]} \\
& +
\sum\limits_{i_1 = 1}^{n_1}
\sum\limits_{i_2 = 1}^{n_2}
\dots
\sum\limits_{i_d = 1}^{n_d}
\left(
\bm S_{n_1}^{-i_1+1} \otimes \dots \otimes \bm S_{n_d}^{-i_d+1}
\right)
\overline{u}_{[i_1, i_2, \dots, i_d]}.
\end{align}
%
Now, we can differentiate above inner product for given multiindex $\bm e$ with respect to $u_{\bm e}$ via
%
\begin{align}
&\frac{\partial}{\partial u_{\bm e}} \langle \bm A, \bm{T}_{(\bm{n},d)}(\bm u) \rangle =\\
    = &\frac{\partial}{\partial u_{\bm e}}
       \sum\limits_{i_1 = 1}^{n_1}
       \sum\limits_{i_2 = 1}^{n_2}
       \dots
       \sum\limits_{i_d = 1}^{n_d}
       \left\langle
       \bm A,
       \bm S_{n_1}^{-i_1} \otimes \dots \otimes \bm S_{n_d}^{-i_d}
       \right\rangle
       u_{[i_1, i_2, \dots, i_d]} =\\
    = &\left\langle
       \bm A,
       \bm S_{n_1}^{-e_1 + 1} \otimes \dots \otimes \bm S_{n_d}^{-e_d + 1}
       \right\rangle.
\end{align}
%
Note that $\bm S_{n_1}^{-e_1 + 1} \otimes \dots \otimes \bm S_{n_d}^{-e_d + 1} = \bm I_{n_1 \cdot \dots \cdot n_d}$ for $e_1 = \dots = e_d = 1$ and in this case above inner product reduces to the trace of $\bm A$. In the other cases the inner product with these specially structured Kronecker products is a summation over diagonals in lower blocks of $\bm A$, whose size is defined by the multilevel block structure. For given $\bm n \in \N^d$ let $f : \N^d \rightarrow \N$ be defined as
\[
f_{\bm n}([i_1, \dots, i_d]) = \prod\limits_{k = 1}^d (2 (n_k - i_k + 1) - \delta_{1,i_k} n_k).
\]
%
Now for some appropriate multiindex $\bm e$ we can also calculate (Note that here we identify the multiindex $\bm e$ with the the tensor of order $d$ which has zeros everywhere except a single $1$ as position $\bm e$.):
\begin{align*}
    \frac{\partial}{\partial u_{\bm e}}
    \langle
        \bm{T}_{(\bm{n},d)}(\bm u),
        \bm{T}_{(\bm{n},d)}(\bm u)
    \rangle
    & = \\
    \frac{\partial}{\partial u_{\bm e}}
    \Big(
    \sum\limits_{\bm e^\prime} &\left[
    \sum\limits_{\bm e^{\prime\prime}}
        \langle \bm T(\bm e^{\prime\prime}), \bm T(\bm e^{\prime})\rangle
            v_{\bm e^{\prime\prime}} v_{\bm e^{\prime}}
    + \sum\limits_{\bm e^{\prime\prime}}
        \langle \bm T(\jmath \bm e^{\prime\prime}), \bm T(\bm e^{\prime})\rangle
            w_{\bm e^{\prime\prime}} v_{\bm e^{\prime}}
    \right] \\
    + \sum\limits_{\bm e^\prime} &\left[
    \sum\limits_{\bm e^{\prime\prime}}
        \langle \bm T(\bm e^{\prime\prime}), \bm T(\jmath \bm e^{\prime})\rangle
            v_{\bm e^{\prime\prime}} w_{\bm e^{\prime}}
    + \sum\limits_{\bm e^{\prime\prime}}
        \langle \bm T(\jmath \bm e^{\prime\prime}), \bm T(\jmath \bm e^{\prime})\rangle
            w_{\bm e^{\prime\prime}} w_{\bm e^{\prime}}
    \right]
    \Big) =\\
    \frac{\partial}{\partial u_{\bm e}}
    \Big(
    \sum\limits_{\bm e^\prime} &\left[
    \sum\limits_{\bm e^{\prime\prime}}
        \langle \bm T(\bm e^{\prime\prime}), \bm T(\bm e^{\prime})\rangle
            v_{\bm e^{\prime\prime}} v_{\bm e^{\prime}}
    + \sum\limits_{\bm e^{\prime\prime}}
        \langle \bm T(\jmath \bm e^{\prime\prime}), \bm T(\jmath \bm e^{\prime})\rangle
            w_{\bm e^{\prime\prime}} w_{\bm e^{\prime}}
    \right]
    \Big) =\\
    \frac{\partial}{\partial u_{\bm e}}
    \Big(
    \sum\limits_{\bm e^\prime} &\left[
        \langle \bm T(\bm e^{\prime}), \bm T(\bm e^{\prime})\rangle
            v_{\bm e^{\prime}}^2
    -   \langle \bm T(\bm e^{\prime}), \bm T(\bm e^{\prime})\rangle
            w_{\bm e^{\prime}}^2
    \right]
    \Big) = 2 f_{\bm n}(\bm e) \overline{u}_(\bm e),
\end{align*}
%
since $f_{\bm n}(\bm e)$ represents the number of occurrences of $u_{\bm e}$ in the multilevel Toeplitz matrix. Again this generalizes above results for the singlelevel case.

Summarizing, we define the operator $\mathfrak{D}_{\bm n, d} : \C^{n_1 \dots n_d \times n_1 \dots n_d} \rightarrow \C^{n_1 \times \dots \times n_d}$ via
\[
\mathfrak{D}_{\bm n, d}(\bm A)
= \frac{\partial}{\partial \bm u}\langle \bm A, \bm T_{\bm n, d}(\bm u)\rangle = \left\langle
   \bm A,
   \bm S_{n_1}^{-e_1 + 1} \otimes \dots \otimes \bm S_{n_d}^{-e_d + 1}
   \right\rangle
.\]

\subsection{Completing the ADMM}

Again, we want to formulate the ADMM iteration in order to approximate a solution to \eqref{ML_ANM}. To this end, we get the augmented Lagrangian as before, which reads as
\begin{align}
   \min_{t,\bm u, \bm x, \bm Z \succeq \bm 0, \bm \Lambda \succeq \bm 0} & \mathcal L(t,\bm u, \bm x, \bm Z , \bm \Lambda ) \label{ML_LAG_ADMM}
\end{align}
where
\begin{align*}
	\mathcal L(t,\bm u, \bm x, \bm Z , \bm \Lambda )
	   = & \frac 12 \Norm{\bm \Gamma \bm x - \bm y}^2
        + \frac{\tau}{2}(t + u_{[1, \dots, 1]})
        + \left\langle
            \bm \Lambda, \bm Z
            - \begin{bmatrix}
                \bm{T}_{(\bm{n},d)}(\bm u) & \bm x \\
                \bm x^\herm & t
            \end{bmatrix}
        \right\rangle \\
        & + \frac{\rho}{2} \Norm{
        \bm Z
        - \begin{bmatrix}
            \bm{T}_{(\bm{n}, d)}(\bm u) & \bm x \\
            \bm x^\herm & t
        \end{bmatrix}}^2.
\end{align*}

With the same arguments and partitioning as above, we rewrite the Lagrangian as
%
\begin{align}\label{ML_LAG_ADMM2}
\mathcal L(t,\bm u, \bm x, \bm Z , \bm \Lambda )
	= &\frac 12 \Norm{\bm \Gamma \bm x - \bm y}^2
    + \frac{\tau}{2}(t + u_{[1, \dots, 1]})
	+ \left\langle
        \bm \Lambda_0, \bm Z_0 - \bm{T}_{(\bm{n},d)}(\bm u)
      \right\rangle \notag \\ &
	+ \langle \bm \lambda_1, \bm z_1 - \bm x \rangle
	+ \langle \bm z_1 - \bm x, \bm \lambda_1 \rangle
	+ \lambda_n \cdot (z_n - t) \notag \\ &
	+ \frac{\rho}{2} \left(
	   \Norm{\bm Z_0 - \bm{T}_{(\bm{n},d)}(\bm u)}^2
		+ 2 \Norm{\bm z_1 - \bm x}^2
		+ (z_n - t)^2
	\right)
\end{align}

As one can see, only the derivative of $\mathcal{L}$ with respect to $\bm u$ is prone to change in the multidimensional case, so we tackle this below. We calculate for some appropriate and fixed multiindex $\bm e$
\[
    \frac{\partial \mathcal{L}}{\partial u_{\bm e}} =
        \frac{\tau}{2} \bm e_{[1, \dots, 1]} - \mathfrak{D}_{\bm n, d}(\bm \Lambda_0 + \rho \bm Z_0)_{\bm e}
    + \rho f_{\bm n}(\bm e) \cdot \overline{\bm u},
\]
which suggests a similar update rule as in the single-dimensional case. There are some things to consider:
\begin{itemize}
    \item I am not sure, how to exactly generalize a single-level Hermitian Toeplitz matrix to more levels. Is each level block supposed to be Hermitian, or does it suffice that the whole matrix is Hermitian. As it is defined right now, the latter is enforced, since we define it recursively.

    \item Above point also makes the derivatives questionable, since these highly depend on the definition of $T$.
\end{itemize}

\section{The Algorithm}

\subsection{Formulation}

\subsection{Speeding up the ADMM}
\begin{itemize}
    \item We use the $\bm U_k$ to roughly diagonalize $T(\bm u_{k + 1})$. Then we use the Gershgorin disk theorem to estimate which
\end{itemize}

\newpage

\subsubsection{Speeding up the Projection on the Positive Cone}

Suppose we are given the iterate $\bm T_k = T(\bm u_k) \in C^{n \times n}$, which is an Hermitian Toeplitz matrix along with its diagonalization $\bm T_k = \bm U_k \bm D_k \bm U_k^\herm$, where each entry of the diagonal matrix $\bm D_k$ is non-negative, but we are in the scenario, where it is very likely that some of them are $0$, since $T_k$ is the result of a projection step of some other matrix $\bm S_k$ onto the positive cone. After each iteration of the algorithm, we have that
\[T(\bm u_{k+1}) = \bm T_{k+1} = \bm T_k + \bm P_{k+1},\]
where $\bm P_k$ is a small pertubation in some matrix norm sense. The goal is now twofold:
\begin{enumerate}
    \item\label{identify} to give a quick decision rule, whether $\bm T_{k+1}$ must be projected onto the positive cone, i.e. decide whether some eigenvalues of $\bm T_{k+1}$ might be negative and
    \item if so to carry out an in some sense selective diagonalization, which only modifies the parts of the spectrum that where identified in \ref{identify}. and makes use of the already and "close enough" $\bm D_k$ and $\bm U_k$ of the last step.
\end{enumerate}

To address the issue in \ref{identify}. we make use of the Gershgorin circle theorem, which states that for each eigenvalue $\lambda$ of the matrix $\bm A$ we have that
\[\vert \lambda - a_{ii}\vert \leqslant \sum\limits_{j \neq i} \vert a_{ij} \vert.\]

If we now set
\[\bm A = \bm U_k^\herm \bm T_{k+1} \bm U_k = \bm D_k + \bm F_{k+1},\]
where again $\bm F_{k+1}$ is small in some matrix norm sense, we have that
\[\vert \lambda - a_{ii}\vert = \vert \lambda - (d_{k,ii} + f_{k+1,ii}) \vert \leqslant \sum\limits_{j \neq i} \vert f_{k+1,ij} \vert = R_i.\]
Since we assumed $\bm F_{k+1}$ to be a small matrix, we know that the resulting Gershgorin disk radii $R_i$ will be small. If now $0 \in [a_{ii} - R_i, a_{ii} + R_i]$ for some $1 \leqslant i \leqslant n$, we must assume that the pertubation $\bm P_k$ altered $\bm T_k$ to become indefinite.

In this case, we would like to apply an algorithm for the projection on the positive cone, which makes use of the matrices known from step $k$ and the fact that $\bm T_{k+1}$ and $\bm T_k$ are close.


==> tex/single_dim.tex <==
% !TEX root = ../main.tex


Following~\cite{bhaskar2013ANDNlinespecest}, the problem we are trying to solve is given by
%
\begin{align}
    \min_{t,\bm u, \bm x}
        \frac 12 \Norm{\bm \Gamma \bm x - \bm y}^2
        + \frac{\tau}{2}(t + \Real{u_1}) \label{eqn:opt_anm} \\
		\text{subject to} \quad
        \begin{bmatrix}
            T(\bm u) & \bm x \\
            \bm x^\herm & t
        \end{bmatrix} \succeq \bm 0, \notag
\end{align}
%
where the matrix $\bm \Gamma$ was introduced in addition to what is in \cite{bhaskar2013ANDNlinespecest}, following the generalized line spectral estimation idea from~\cite{heckel2017gen_line_spec_est}. The operator $T(\bm u)$ maps a complex vector $\bm u$ onto a Hermitian symmetric Toeplitz matrix via
%
\begin{align}\label{toep_single}
   T(\bm u) =
        \begin{bmatrix}
	        \Real{u_1} & u_2 & u_3 & \ldots & u_n \\
			\Conj{u}_2 & \Real{u_1} & u_2 & \ldots & u_{n-1} \\
			\vdots & \vdots & \vdots & \ddots & \vdots \\
			\Conj{u}_n & \Conj{u}_{n-1} & \Conj{u}_{n-2} & \ldots & \Real{u_1}.
		\end{bmatrix}
\end{align}
%
Note that the $\Real{u_1}$ is missing in \cite{bhaskar2013ANDNlinespecest}, however, is necessary to make sure that $T(\bm u)$ is Hermitian symmetric.
As explained in \cite{bhaskar2013ANDNlinespecest}, an ADMM version of \eqref{eqn:opt_anm} is given by
%
\begin{align}
    \min_{
        t,
        \bm u,
        \bm x,
        \bm Z \succeq \bm 0,
        \bm \Lambda \succeq \bm 0
    }
    \mathcal L(t,\bm u, \bm x, \bm Z , \bm \Lambda)
    \label{eqn:augmented_lagrangian}
\end{align}
where the so called augmented Lagrangian reads as
\begin{align}
	\mathcal L(t,\bm u, \bm x, \bm Z , \bm \Lambda )
	= &\frac 12 \Norm{\bm \Gamma \bm x - \bm y}^2
    + \frac{\tau}{2}(t + \Real{u_1})
	+ \left\langle
        \bm \Lambda, \bm Z
        - \begin{bmatrix}
            T(\bm u) & \bm x \\
            \bm x^\herm & t
        \end{bmatrix}
    \right\rangle \\
	+ &\frac{\rho}{2} \Norm{
        \bm Z
        -\begin{bmatrix}
            T(\bm u) & \bm x \\
            \bm x^\herm & t
        \end{bmatrix}
    }^2.
\end{align}
%
Note that $\langle \bm A, \bm B \rangle = \Tr{\bm A^\herm \bm B} \in \R$ for Hermitian matrices $\bm A, \bm B$. The Hermitian symmetry is enforced by partitioning $\bm Z$ and $\bm \Lambda$ as
%
\begin{align}
  \bm Z = \begin{bmatrix} \bm Z_0 & \bm z_1 \\ \bm z_1^\herm & z_n \end{bmatrix}
	\quad
	\bm \Lambda = \begin{bmatrix} \bm \Lambda_0 & \bm \lambda_1 \\ \bm \lambda_1^\herm & \lambda_n \end{bmatrix}.
\end{align}
%
This allows to rewrite the Lagrangian as
%
\begin{align}
\mathcal L(t,\bm u, \bm x, \bm Z , \bm \Lambda )
	& = \frac 12 \Norm{\bm \Gamma \bm x - \bm y}^2 + \frac{\tau}{2}(t + \Real{u_1})
	+ \left\langle \bm \Lambda_0, \bm Z_0 - T(\bm u)\right\rangle \\
	&+ \langle \bm \lambda_1, \bm z_1 - \bm x \rangle
	+ \langle \bm z_1 - \bm x, \bm \lambda_1 \rangle
	+ \lambda_n \cdot (z_n - t) \notag \\
    &+ \frac{\rho}{2} \left(
	   \Norm{\bm Z_0 - T(\bm u)}^2
		+ 2 \Norm{\bm z_1 - \bm x}^2
		+ (z_n - t)^2
	\right)
\end{align}
%
To solve \eqref{eqn:augmented_lagrangian} via ADMM, we require the gradients with respect to all the arguments. This document provides a rigorous derivation of these gradients.

\subsection{Ingredients}
\subsubsection{Wirtinger derivatives}
%
Though $\mathcal L$ is naturally real-valued, most of its parameters are indeed complex. Therefore, we need a proper notion of complex derivatives. We follow the Wirtinger calculus idea which
%for the special case of functions $f: \C^n \mapsto \R$
defines derivatives of a function $f(\bm x)$ with respect to its complex argument $\bm x$ via
%
\begin{align}
   \frac{\partial f}{\partial \bm x} & = \frac 12 \left( \frac{\partial f}{\partial \bm y} - \jmath \frac{\partial f}{\partial \bm z} \right) \notag \\
	\frac{\partial f}{\partial \Conj{\bm x}} & = \frac 12 \left( \frac{\partial f}{\partial \bm y} + \jmath \frac{\partial f}{\partial \bm z} \right), \notag
\end{align}
%
where $\bm y = \Real{\bm x}$ and $\bm z = \Imag{\bm x}$. Note that for $f(x) = \Conj{x} =  y-\jmath z$ we obtain
%
\begin{align}
    \frac{\partial \Conj{x}}{\partial x} = \frac 12 \left( \frac{\partial y-\jmath z}{\partial  y} - \jmath \frac{\partial  y-\jmath z}{\partial  z} \right)
		= \frac 12 \left(1 - \jmath (-\jmath) \right) = 0. \label{eqn:wder_xxbar}
\end{align}
%
For this reason, in Wirtinger derivatives we can more or less treat $x$ and $\Conj{x}$ as independent variables.
%
The functions we are interested in are of the form $f: \C^n \mapsto \R$. For these, we obviously have
%
\begin{align}
   \frac{\partial f}{\partial \bm x} = \Conj{\frac{\partial f}{\partial \Conj{\bm x}}}.
\end{align}
%
Therefore, to find stationary points of $f$ where the derivative vanishes, we can either consider the derivative with respect to $\bm x$ of $\Conj{\bm x}$, the result is the same.
%
%
%
%
\subsubsection{Inner Products and Norms}

We will make use of the following rules
%
\begin{align}
 \frac{\partial \langle \bm b, \bm a\rangle}{\partial \Conj{\bm b}} =
 \frac{\partial \bm{b}^\herm \bm a}{\partial \Conj{\bm b}} & = \bm a \label{eqn:wder_lin} \\
\frac{\partial \langle \bm a, \bm b\rangle}{\partial \Conj{\bm b}} =
  \frac{\partial \bm{a}^\herm \bm b}{\partial \Conj{\bm b}} & = \bm 0 \label{eqn:wder_lin_c} \\
   \frac{\partial \Norm{\bm{A} \cdot \bm{b} - \bm{c}}^2}{\partial \Conj{\bm{b}}}
	& = \frac{\partial}{\partial \Conj{\bm b}} \left( \bm b^\herm \bm A^\herm \bm A \bm b - \bm b^\herm \bm A^\herm \bm c - \bm c^\herm \bm A \bm b + \bm c^\herm \bm c\right) \\
	& = \bm A^\herm \bm A \bm b - \bm A^\herm \bm c
	= \bm A^\herm (\bm A \bm b - \bm c) \label{eqn:wder_norm}
\end{align}
%
where \eqref{eqn:wder_lin_c} follows from \eqref{eqn:wder_xxbar}
and \eqref{eqn:wder_norm} follows from expanding $\Norm{\bm{x}}^2 = \bm{x}^\herm \bm{x}$ and then applying \eqref{eqn:wder_lin} and \eqref{eqn:wder_lin_c}.

\subsection{The Hermitian Toeplitz Operator}

We also need derivatives involving the operator $T(\bm u)$, e.g., $\frac{\partial}{\partial \bm u} \langle \bm A, T(\bm u)\rangle$ for a Hermitian matrix $\bm A$. The original references do not discuss this step in detail but seem to argue that we can find the derivative via its adjoint according to
%
\begin{align}
   \frac{\partial}{\partial \bm u} \langle \bm A, T(\bm u)\rangle
	= \frac{\partial}{\partial \bm u} \langle T^*(\bm A), \bm u\rangle
	= T^*(\bm A),
\end{align}
%
where $T^*$ is the adjoint operator. However, this is problematic since due to the conjugations in $T$, it
%as discussed above, to make sure $T(\bm u)$ is Hermitian, we need to take the real part of its first argument. Therefore, $T$
is not $\C$-linear and it does not have an adjoint with respect to $\C^n$ (In fact there exists no non-trivial $\C$-linear operator from $\C^n$ to Hermitian matrices).

It is therefore easier to expand the derivatives using the natural $\R^{2n}$ embedding via $\bm u = \bm v + \jmath \bm w$. For a Hermitian matrix $\bm A$, we can write
%
\begin{align*}
   \langle \bm A, T(\bm u)\rangle
	& = \langle \bm A, T(\bm v + \jmath \bm w)\rangle \\
	& =  \langle \bm A, T(\bm v)\rangle +  \langle \bm A, T(\jmath \bm w)\rangle \\
	& = \sum_{i=1}^n \langle \bm A, T(\bm e_i)\rangle v_i
	 + \sum_{i=1}^n \langle \bm A, T(\jmath \bm e_i)\rangle w_i,
\end{align*}
%
where $\bm e_i$ is the $i$-th cartesian unit vector (having a one on its $i$-th position and zeros elsewhere).
This allows us to compute the Wirtinger derivative via
%
\begin{align}
   \frac{\partial}{\partial u_k}\langle \bm A, T(\bm u)\rangle = \frac 12 \Big( \langle \bm A, T(\bm e_k)\rangle -\jmath \langle \bm A, T(\jmath \bm e_k)\rangle \Big)
\end{align}

To proceed let us define the shift matrix $\bm{S}$ via
%
\begin{align}
  \bm S = \begin{bmatrix}
	0 & 1 & 0 & \ldots & 0 \\
	0 & 0 & 1 & \ldots & 0 \\
	\vdots & \ddots & \ddots & \ddots & \vdots \\
	0 & 0 & 0 & \ldots & 1 \\
	0 & 0 & 0 & \ldots & 0
	\end{bmatrix},
\end{align}
%
so $\bm{S}_{(k,\ell)} = 1$ if $\ell-k=1$. Note that $\bm{S}^d$ has ones on its $d$-th upper diagonal and zeros elsewhere. Moreover, for $d > 0$ we define $\bm S^{-d} = {\bm S^d}^\trans$. With the help of $\bm{S}$, we can write
%
\begin{align}
   T(\bm{e}_k) & = \begin{cases}
	    \bm S^0 = \bm I_n & k = 1 \\
	    \bm S^{k-1} + \bm S^{-k+1} & k > 1
		\end{cases} \\
	 T(\jmath \bm{e}_k) & = \begin{cases}
	    \bm 0 & k = 1 \\
	    \jmath \bm S^{k-1} -\jmath \bm S^{-k+1} & k > 1
		\end{cases}
\end{align}
%
Therefore, we have
%
\begin{align}
\frac{\partial}{\partial u_1}\langle \bm A, T(\bm u)\rangle & = \frac 12 \langle \bm A, \bm I_n\rangle = \frac 12 \Tr{\bm A^\herm} = \Tr{\bm A} \quad \mbox{and for $k>1$:} \notag \\
\frac{\partial}{\partial u_k}\langle \bm A, T(\bm u)\rangle
&=	\frac 12\left(
	\langle \bm A, \bm S^{k-1} + \bm S^{-k+1}\rangle
	- \jmath
	\langle \bm A, \jmath \bm S^{k-1} -\jmath \bm S^{-k+1}\rangle
	\right) \notag \\
	& =
	\frac 12
	\langle \bm A, \bm S^{k-1} + \bm S^{-k+1}
	+\bm{S}^{k-1}-\bm S^{-k+1}
	\rangle
	= \langle \bm A, \bm S^{k-1} \rangle
\end{align}
%
To simplify the notation we define an operator $\mathcal D$ via
%
\begin{align}
   \mathcal D(\bm{A})
        & = \begin{bmatrix}
            \frac 12 \Tr{\bm A} \\
            \langle \bm A, \bm{S} \rangle \\
            \langle \bm A, \bm{S}^2 \rangle \\
            \vdots \\
            \langle \bm A, \bm{S}^{n-1} \rangle
		\end{bmatrix},
\end{align}
which satisfies
\begin{align}
		\frac{\partial}{\partial \bm{u}}
		\langle \bm A, T(\bm u)\rangle & = \mathcal D(\bm{A}).
		\label{eqn:deriv_innerp_Tofu}
\end{align}
%
Note that since for Hermitian matrices $\bm A$ we have $\langle \bm A, T(\bm u)\rangle$, it also holds that
$\langle \bm A, T(\bm u)\rangle = \langle T(\bm u), \bm A\rangle$ and therefore
$\frac{\partial}{\partial \bm{u}} \langle T(\bm u), \bm A\rangle = \mathcal D(\bm{A})$ as well. Note also that $\langle \bm A, \bm S^k\rangle$ is equivalent to summing the $k$-th \textbf{lower} diagonal of $\bm A$, because $\langle \bm A, \bm B \rangle = \Tr{\bm A^\herm \cdot \bm B}$ and $\bm A$ is Hermitian.

We can then also compute $\mathcal D( T(\bm u))$ and obtain
%
\begin{align}
   \mathcal D( T(\bm u))
	= \begin{bmatrix}
	  \frac 12 n \cdot \Real{u_1} \\
        (n-1) \cdot \Conj{u_2} \\
        (n-2) \cdot \Conj{u_3} \\
		\vdots \\
        1 \cdot \Conj{u_n}
		\end{bmatrix}
		= \bm W \cdot \Conj{\tilde{\bm u}}, \label{eqn:doftofu}
\end{align}
%
where $\bm W = \frac 12 \Diag{n, 2(n-1), 2(n-2), \ldots, 2}$ and $\tilde{\bm u} = [\Real{u_1}, u_2, ..., u_n]^\trans$ which is equal to $\bm u$ if its first element is real-valued.

Our final ingredient is the Frobenius norm term including $T(\bm u)$. To evaluate it, we will establish the rule
%
\begin{align}
  \frac{\partial}{\partial \bm u}
  \langle T(\bm u), T(\bm u)\rangle
	= 2 \Conj{\mathcal D(T(\bm u))}. \label{eqn:der_tofu_quad}
\end{align}
%
To show~\eqref{eqn:der_tofu_quad}, note that $\langle T(\bm u), T(\bm u)\rangle = \Norm{T(\bm u)}^2$, which we can write as
%
\begin{align}
   \langle T(\bm u), T(\bm u)\rangle
    & = \Norm{T(\bm u)}^2
    = \sum_{n_1,n_2} \left|[T(\bm u)]_{n_1,n_2}\right|^2 \notag \\
	& = n \cdot \Real{u_1}^2 + 2(n-1)|u_2|^2 + 2(n-2)|u_3|^2 + \ldots + 2|u_n|^2 \notag \\
	& = n \cdot v_1^2 + 2\sum_{\ell=2}^{n}(n-\ell+1)(v_\ell^2 + w_\ell^2).
\end{align}
%
Therefore, the Wirtinger derivative becomes
%
\begin{align}
  \frac{\partial}{\partial u_k} \langle T(\bm u), T(\bm u)\rangle
	& = \frac 12 \left( \frac{\partial}{\partial v_k} - \jmath \frac{\partial}{\partial w_k} \right)
	\left(n \cdot v_1^2 + 2\sum_{\ell=2}^{n}(n-\ell+1)(v_\ell^2 + w_\ell^2) \right) \notag \\
	& = \frac 12 \cdot \begin{cases}
	   2 n v_1 & k = 1 \\
		4(n-k+1) (v_k - \jmath  w_k) & k>1
	\end{cases} \notag \\
	& = 2 \cdot \begin{cases}
	   \frac 12 n \Real{u_1} & k = 1 \\
		 (n-k+1) \Conj{u}_k & k>1,
	\end{cases}
\end{align}
%
which shows \eqref{eqn:der_tofu_quad}. Based on \eqref{eqn:der_tofu_quad} we can then differentiate norms via
%
\begin{align}
  \frac{\partial}{\partial \bm u}  \Norm{\bm{A} - \bm{T}(\bm u)}^2
	& = \frac{\partial}{\partial \bm u} \langle \bm{A}-\bm{T}(\bm u),\bm{A}-\bm{T}(\bm u)\rangle \notag \\
	& = \frac{\partial}{\partial \bm u} \left(
	   \langle\bm{A},\bm{A}\rangle - \langle \bm{A},{T}(\bm u) \rangle
		- \langle {T}(\bm u),\bm{A} \rangle
		+ \langle {T}(\bm u), {T}(\bm u) \rangle \right) \notag \\
	& = - 2\mathcal D(\bm{A}) + 2 \Conj{\mathcal D(T(\bm u))} \label{eqn:deriv_fronorm_Tofu}
\end{align}

\subsection{Derivatives}

With the necessary tools established we can now compute the derivatives of the augmented Lagrangian \eqref{eqn:augmented_lagrangian} to find he ADMM iteration rules.

Starting with the scalar $t$, we obtain
%
\begin{align}
   \frac{\partial \mathcal L}{\partial t}
	= \frac{\tau}{2} - \lambda_n - \rho(z_n - t)
	= 0 \; \Leftrightarrow \; t = z_n + \frac{1}{\rho}\left(\lambda_n - \frac{\tau}{2}\right). \label{eqn:upddate_t}
\end{align}
%
For $\bm x$, using \eqref{eqn:wder_lin}, \eqref{eqn:wder_lin_c}, and \eqref{eqn:wder_norm}, we find
%
\begin{align}
   \frac{\partial \mathcal L}{\partial \Conj{\bm x}}
	  & = \frac 12  \bm{\Gamma}^\herm \left(\bm{\Gamma} \bm x - \bm y\right) - \bm \lambda_1 - \rho \left( \bm z_1 - \bm x\right) = \bm 0 \; \Leftrightarrow \notag \\
	\left( \frac 12 \bm \Gamma^\herm \bm \Gamma + \rho \bm I_n\right) \cdot \bm x
	& = \frac 12 \bm \Gamma^\herm \bm y
	+ \bm \lambda_1 + \rho \bm z_1 \notag \\
	\bm x & = \left( \bm \Gamma^\herm \bm \Gamma + 2\rho\bm I_n\right)^{-1} \left( \bm\Gamma^\herm \bm y + 2 \bm \lambda_1 + 2 \rho \bm z_1 \right). \label{eqn:upddate_x}
\end{align}
%
Moreover, for $\bm u$, using \eqref{eqn:deriv_innerp_Tofu}, \eqref{eqn:deriv_fronorm_Tofu} and  we get
%
\begin{align*}
   \frac{\partial \mathcal L}{\partial {\bm u}}
	& = \frac{\partial }{\partial {\bm u}}
	\left(
        \frac{\tau}{2} \Real{u_1}
        - \left\langle \bm \Lambda_0, T(\bm u)\right\rangle
        + \frac{\rho}{2} \Norm{\bm Z_0 - T(\bm u)}^2
    \right) \notag \\
    & = \frac{\tau}{2} \bm e_1 - \mathcal D(\bm \Lambda_0)
    + \frac{\rho}{2} \left(-2\mathcal D(\bm Z_0)
    + 2 \Conj{\mathcal D(T(\bm u))}\right) \notag \\
    & = \frac{\tau}{2} \bm e_1 -\mathcal D(\bm \Lambda_0 + \rho \bm Z_0)
    + \rho \bm W \tilde{\bm u}
\end{align*}
Equating the last expression above to $\bm 0$ yields
\begin{align}
    \tilde{\bm u}
        = \bm{W}^{-1} \cdot
        \left(
            \mathcal D\left(\frac{1}{\rho}\bm \Lambda_0 + \bm{Z}_0
        \right)
        - \frac{\tau}{2\rho} \bm e_1 \right)
        \label{eqn:upddate_u}
\end{align}

\subsection{Comparison to \cite{bhaskar2013ANDNlinespecest} and \cite{li2016offgridlinespectrumdenoising}}

If we compare these update rules to the ones stated in \cite{bhaskar2013ANDNlinespecest} (Appendix~E of its arxiv version), we find:
\begin{itemize}
	\item The update rule for $t$ is identical.
	\item The update rule for $\bm x$ is identical if we set $\bm \Gamma = \bm I$.
	\item In \cite{bhaskar2013ANDNlinespecest} the matrix $\bm{W}^{-1}$ is defined as having the vector $[\frac{1}{n}, \frac{1}{2(n-1)}, \frac{1}{2(n-2)}, ..., \frac{1}{2}]$ on its main diagonal. In our update rule, $\bm{W}$ has $[\frac{2}{n}, \frac{1}{n-1}, \frac{1}{n-2}, ..., 1]$ on its main diagonal, i.e., it is a factor 2 larger.
\end{itemize}

We can also compare it to the MMV version in \cite{li2016offgridlinespectrumdenoising} by setting the number of measurement vectors ($L$) to one. We then find:
\begin{itemize}
	\item The update rule for $t$ is identical.
	\item The update rule for $\bm x$ is identical if we set $\bm \Gamma = \bm I$.
	\item The update rule for $\bm u$ differs in four aspects:
	\begin{enumerate}
		\item The term $\frac{\tau}{2} \bm{e}_1$ is replaced by $\frac{\tau}{2} n \bm{e}_1$. Note that $n$ is not the number of measurement vectors but the problem dimension.
		\begin{itemize}
			\item {\em New piece of information: the source of inconsistency has been found: \cite{li2016offgridlinespectrumdenoising} defines their atoms with a factor $1/\sqrt{n}$ in front. This is why instead of $1/n \cdot \Tr{T(\bm u)} = u_1$ they have $\Tr{T(\bm u)} = n\cdot u_1$, which brings a factor $n$ here.}
		\end{itemize}
		\item The matrix $\bm{W}^{-1}$ (in \cite{li2016offgridlinespectrumdenoising} called $\bm \Upsilon$ is stated as having $[\frac{1}{n}, \frac{1}{n-1}, \frac{1}{n-2}, ..., 1]$ on its main diagonal. Hence, it disagrees to our $\bm{W}^{-1}$ in the first element (which we derived as $\frac{2}{n}$).
		\item In \cite{li2016offgridlinespectrumdenoising} the operator $\mathcal D$ is explicitly described as summing the upper diagonals, like we defined it here. However, it differs from our operator in the first element where we carry a factor $1/2$. It may sound like this is the explanation for the difference regarding $\bm{W}$, however, note that $\bm{W}^{-1}$ also scales the $\tau/2 \cdot \bm{e}_1$ term.
		\item While \cite{li2016offgridlinespectrumdenoising} seems to agree to our derivation regarding the conjugates this is actually not the case since they define their operator $T(\bm u)$ differently, namely, having $\bm u$ as the first column (whereas \cite{bhaskar2013ANDNlinespecest} and we have it as the first row). Since $T(\bm u)$ is Hermitian this is like replacing $\bm u$ by $\Conj{\bm u}$. Therefore, \cite{li2016offgridlinespectrumdenoising} and \cite{bhaskar2013ANDNlinespecest} agree in terms of the conjugation and it is inconsistent with our derivation. Numerical evidence suggests that they are right and we are wrong but I don't see why.
	\end{enumerate}
\end{itemize}


\subsection{Completing the ADMM}

The ADMM iterations proceed by alternating the following three steps
%
\begin{align}
   (t, \bm{x}, \bm{u}) & = \arg \min_{t, \bm{x}, \bm{u}} \mathcal L(t, \bm{x}, \bm{u},\bm{\Lambda},\bm{Z})
	\label{eqn:update_txu} \\
	\bm{Z} & = \arg \min_{\bm Z \succeq \bm 0} \mathcal L(t, \bm{x}, \bm{u},\bm{\Lambda},\bm{Z})
	\label{eqn:update_Z} \\
	\bm{\Lambda} & \leftarrow \bm{\Lambda} + \rho \cdot\left(\bm{Z} - \begin{bmatrix} T(\bm u) & \bm x \\ \bm x^\herm & t \end{bmatrix}\right).
	\label{eqn:update_Lambda}
\end{align}
%
{\em Note: I'm not sure how to properly derive \eqref{eqn:update_Lambda}. In the original ADMM paper, it is stated that the dual ascent is $\bm \lambda \leftarrow \bm \lambda + \rho (\bm{A}\bm{x}-\bm{b})$ and this rule comes from there. However, changes have to be made since the vector $\bm{\lambda}$ becomes a Hermitian positive definite matrix $\bm \Lambda$ in our case.}

The update rules for performing \eqref{eqn:update_txu} (with respect to the variables $t, \bm x, \bm u$ separately) are given in \eqref{eqn:upddate_t}, \eqref{eqn:upddate_x}, and \eqref{eqn:upddate_u}, respectively. Also, \eqref{eqn:update_Lambda} can be implemented directly. To carry out \eqref{eqn:update_Z} we again consider a gradient and obtain
%
\begin{align}
  \frac{\partial \mathcal L}{\partial \Conj{\bm Z}}
	= \frac{\partial}{\partial \Conj{\bm Z}}
	\left(\langle\bm \Lambda, \bm Z\rangle
	+ \frac{\rho}{2} \Norm{\bm Z - \begin{bmatrix} T(\bm u) & \bm x \\ \bm x^\herm & t \end{bmatrix}}^2
	\right)
	= \bm \Lambda
	+ \frac{\rho}{2} \left(\bm Z - \begin{bmatrix} T(\bm u) & \bm x \\ \bm x^\herm & t \end{bmatrix}
	\right),
\end{align}
%
which suggests the update rule
%
\begin{align}
  \bm{Z} = \begin{bmatrix} T(\bm u) & \bm x \\ \bm x^\herm & t \end{bmatrix} - \frac{2}{\rho}\bm\Lambda.
\end{align}
%
However, this matrix is not guaranteed to be positive semidefinite. This issue can be solved by projecting the above update onto the positive semidefinite cone (via truncation of the negative eigenvalues) \cite{bhaskar2013ANDNlinespecest}.

{\em Notes:
\begin{itemize}
	\item I'm not sure how rigorous this derivation is: the gradients are correct for unstructured matrices so they ignore the Hermitian symmetry.

	\item In \cite{bhaskar2013ANDNlinespecest} and \cite{li2016offgridlinespectrumdenoising}, a rule like \eqref{eqn:update_Z} is given, however, it differs from ours in that the factor $\frac{2}{\rho}$ is stated as $\frac{1}{\rho}$ both in \cite{bhaskar2013ANDNlinespecest} as well as \cite{li2016offgridlinespectrumdenoising}. No idea why. Numerical evidence suggests the $\frac{2}{\rho}$ might be wrong as it leads to slightly oscillating estimates, which does not happen for $\frac{1}{\rho}$.
\end{itemize}
}

